Learning Constrained Markov Decision Processes With Non-stationary Rewards and Constraints

In constrained Markov decision processes (CMDPs) with adversarial rewards and constraints, a well-known impossibility result prevents any algorithm from attaining both sublinear regret and sublinear constraint violation, when competing against a best-in-hindsight policy that satisfies constraints on average. In this paper, we show that this negative result can be eased in CMDPs with non-stationary rewards and constraints, by providing algorithms whose performances smoothly degrade as non-stationarity increases. Specifically, we propose algorithms attaining $\tilde{\mathcal{O}} (\sqrt{T} + C)$ regret and positive constraint violation under bandit feedback, where $C$ is a corruption value measuring the environment non-stationarity. This can be $\Theta(T)$ in the worst case, coherently with the impossibility result for adversarial CMDPs. First, we design an algorithm with the desired guarantees when $C$ is known. Then, in the case $C$ is unknown, we show how to obtain the same results by embedding such an algorithm in a general meta-procedure. This is of independent interest, as it can be applied to any non-stationary constrained online learning setting.

==> Arxiv/abstract.tex <==
\begin{abstract}
 	In \emph{constrained Markov decision processes} (CMDPs) with \emph{adversarial} rewards and constraints, a well-known impossibility result prevents any algorithm from attaining both sublinear regret and sublinear constraint violation, when competing against a best-in-hindsight policy that satisfies constraints on average.
 	%
 	In this paper, we show that this negative result can be eased in CMDPs with \emph{non-stationary} rewards and constraints, by providing algorithms whose performances smoothly degrade as non-stationarity increases.
 	%
 	Specifically, we propose algorithms attaining $\tilde{\mathcal{O}} (\sqrt{T} + C)$ regret and \emph{positive} constraint violation under \emph{bandit} feedback, where $C$ is a corruption value measuring the environment non-stationarity.
 	%
 	This can be $\Theta(T)$ in the worst case, coherently with the impossibility result for adversarial~CMDPs.
 	%
 	First, we design an algorithm with the desired guarantees when $C$ is known.
 	%
 	Then, in the case $C$ is \emph{unknown}, we show how to obtain the same results by embedding such an algorithm in a general \emph{meta-procedure}.
 	%
 	This is of independent interest, as it can be applied to \emph{any} non-stationary constrained online learning setting.
\end{abstract}

==> Arxiv/c_known.tex <==
\section{Learning when $C$ is known: More optimism is all you need}
\label{sec: known_c}


We start studying the case in which the learner \emph{knows} the adversarial corruption $C$.
%
We propose an algorithm (called \texttt{NS-SOPS}, see also Algorithm~\ref{alg:NS_UCSPS}), which adopts a suitably-designed UCB-like approach encompassing the adversarial corruption $C$ in the confidence bounds of rewards and constraint costs.
%
This effectively results in ``boosting'' the \emph{optimism} of the algorithm, and it allows to achieve regret and positive constraint violation of the order of $\tilde{\mathcal{O}}(\sqrt{T}+C)$.
%
The \texttt{NS-SOPS} algorithm is also a crucial building block in the design of our algorithm for the case in which the adversarial corruption $C$ is \emph{not} known, as we show in the following section.
%
%
%
%In the following section, we assume that the learner knows the true corruption value $C$. Thus, we propose an algorithm which, encompassing the aforementioned quantity in its optimistic estimated of the environment, achieves the desired regret and violations bounds.



\begin{comment}

\subsection{Confidence intervals}
\label{sec: confidence}


To deal with the lack of knowledge about the transition probabilities $P$, we build a transition confidence set for each episode $t$, namely, $\mathcal{P}_t$ following \cite{JinLearningAdversarial2019}.
We define the empirical transition function up to episode $t\in[T]$ as $
	\overline{P}_t(x'|x,a):=\frac{M_t(x'|x,a)}{\max\{1,N_t(x,a)\}},$
where $M_t(x'|x,a)$ and $N_t(x,a)$ are respectively the total number of visit at the beginning of episode $t$ of couple $(x,a)$ and triplet $(x,a,x')$. 
The confidence set for episode $t$ is defined as:
\begin{equation}
	\label{def: conf int P}
	\mathcal{P}_t := \left\{\widehat{P}:\lvert\overline{P}_t(x'|x,a)-\widehat{P}(x'|x,a)\rvert\le \epsilon_t(x'|x,a),\quad \forall(x,a,x') \in X \times A \times X^\prime\right\},
\end{equation}
where $\epsilon_t(x'|x,a)$ is defined as
$
	\epsilon_t(x'|x,a):= 2 \sqrt{\frac{\overline{P}_t(x'|x,a) \ln\left(\frac{T|X||A|}{\delta} \right) }{\max\{1,N_t(x,a)-1\}}}+\frac{14\ln\left(\frac{T|X||A|}{\delta} \right)}{3\max\{1,N_t(x,a)-1\}},
$
with $\delta \in (0,1).$
%We will refer to the event $P\in \mathcal{P}_t$ for all episodes $t \in [T]$, which holds with probability at least $1-4\delta$,
%as $\mathcal{E}_{P}$.

To deal with the partial feedback we build estimators both for the reward functions and for the cost constraints. Precisely, in order to tackle the corruption of the environment, we build \emph{enlarged} confidence sets as follows.
First, we estimate the empirical reward function as follows:
\begin{equation}
	\label{eq:r estimator}
	\widehat{r}_{t}(x,a):= \frac{1}{\max\{N_t(x,a),1\}}\underset{\tau \in [t]}{\sum}\mathbb{I}_\tau(x,a)r_{\tau}(x,a).
\end{equation}
where $\mathbb{I}_t(x,a)=1$ if and only if $(x,a)$ is visited during episode $t$, and $\mathbb{I}_t(x,a)=0$ otherwise.
Similarly, we build the unbiased estimator $\widehat{G}_t$, and referring to its $i$-th element as $\widehat{g}_{t,i}$, define: 
\begin{equation}
	\label{eq:G estimator}
	\widehat{g}_{t,i}(x,a):= \frac{1}{\max\{N_t(x,a),1\}}\underset{\tau \in [t]}{\sum}\mathbb{I}_\tau(x,a)g_{\tau,i}(x,a).
\end{equation}
We associate to the aforementioned estimators their \emph{enlarged} confidence interval $\phi_t(x,a)$ (for the rewards) and $\xi_t(x,a)$ (for the constraints cost), respectively. Precisely,
for the rewards, we have:
\begin{equation*} 
	\xi_t(x,a)= \min\left\{1,\sqrt{\frac{1}{2 \max\{N_t(x,a),1\}}\ln\left( \frac{2mT|X||A|}{\delta}\right) }+\frac{{C}}{\max\{N_t(x,a),1\}}+\frac{{C}}{T}\right\},
\end{equation*} 
while for the constraints,
\begin{equation*}
	\phi_t(x,a):= \min\left\{1,\sqrt{\frac{1}{2 \max\{N_t(x,a),1\}}\ln\left( \frac{2T|X||A|}{\delta}\right) }+\frac{C}{\max\{N_t(x,a),1\}}+\frac{C}{T}\right\}.
\end{equation*}
Intuitively, the first term of the interval derives from the Azuma-Hoeffding inequality, the second terms encompasses the non-stationarity of the environments, while the third term bound the deviation from the average reward/cost in hindsight and the non-corrupted one.
We refer to Appendix~\ref{app:confidence} for the complete results related to the confidence sets.

\end{comment}





\subsection{\texttt{NS-SOPS}: non-stationary safe optimistic policy search}

% \stradi{l'algoritmo è in parte simile a quello del Pirotta, lo diciamo?}

Algorithm~\ref{alg:NS_UCSPS} provides the pseudocode of the \emph{non-stationary safe optimistic policy search} (\texttt{NS-SOPS} for short) algorithm.
%
The algorithm keeps track of suitably-defined confidence bounds for transition probabilities, rewards, and constraint costs.
%
At each episode $t \in [T]$, the algorithm builds a confidence set $\mathcal{P}_t$ for the transition function $P$ by following the same approach as~\citet{JinLearningAdversarial2019} (see Appendix~\ref{app:auxiliary} for its definition).
%
Instead, for rewards and constraint costs, the algorithm adopts novel \emph{enlarged} confidence bounds, which are suitably designed to tackle non-stationarity.
%
Given $\delta \in (0,1)$, by letting $N_t(x,a)$ be the total number of visits to the state-action pair $(x,a) \in X \times A$ up to episode $t$ (excluded), the confidence bound for the reward $r_t(x,a)$ is:
%
\begin{equation*}
\phi_t(x,a) \coloneqq \min\left\{1,\sqrt{\frac{\ln\left( \nicefrac{2T|X||A|}{\delta}\right)}{2 \max\{N_t(x,a),1\}} }+\frac{C}{\max\{N_t(x,a),1\}}+\frac{C}{T}\right\},
\end{equation*}
while the confidence bound for the constraint costs $g_{t,i}(x,a)$ is defined as:
\begin{equation*} 
\xi_t(x,a) \coloneqq \min\left\{1,\sqrt{\frac{\ln\left( \nicefrac{2mT|X||A|}{\delta}\right)}{2 \max\{N_t(x,a),1\}} }+\frac{{C}}{\max\{N_t(x,a),1\}}+\frac{{C}}{T}\right\}.
\end{equation*} 
%
Intuitively, the first term in the expressions above is derived from Azuma-Hoeffding inequality, the second term allows to deal with the non-stationarity of rewards and constraint costs, while the third term is needed to bound how much the average reward vector $\overline{r}$ and the average constraint costs $[\overline{G}]_i$ differ from their ``fictitious'' non-corrupted counterparts $r^\circ$ and $g^\circ$, respectively.   
%
%bound the deviation from the average reward/cost in hindsight and the non-corrupted one.





Algorithm~\ref{alg:NS_UCSPS} also computes empirical rewards and constraint costs.
%
At each episode $t \in [T]$, for any state-action pair $(x,a) \in X \times A$ and constraint $i \in [m]$, these are defined as follows:
\begin{equation*}
	\widehat{r}_{t}(x,a) \coloneqq \frac{\sum_{\tau \in [t]}\mathbb{I}_\tau(x,a)r_{\tau}(x,a) }{\max\{N_t(x,a),1\}}\quad \text{and} \quad \widehat{g}_{t,i}(x,a) \coloneqq \frac{\sum_{\tau \in [t]}\mathbb{I}_\tau(x,a)g_{\tau,i}(x,a)}{\max\{N_t(x,a),1\}},
\end{equation*}
where $\mathbb{I}_\tau(x,a)=1$ if and only if $(x,a)$ is visited during episode $\tau$, while $\mathbb{I}_\tau(x,a)=0$ otherwise.
%
For ease of notation, we let $\widehat{G}_t \in [0,1]^{|X \times A| \times m}$ be the matrix with components $\widehat{g}_{t,i}(x,a) $.
%
We refer the reader to Appendix~\ref{app:confidence} for all the technical results related to confidence bounds.


		\begin{algorithm}[]
			\caption{\texttt{NS-SOPS}}
			\label{alg:NS_UCSPS}
			\begin{algorithmic}[1]
				\Require $C$, $\delta \in (0,1)$
				%				\State Initialize 
				%				$N_0(x,a)=M_0(x'|x,a)=0,~ \xi_0(x,a)=\phi_0(x,a)=\epsilon_0(x'|x,a)=1,$ $ \forall(x,a,x')\in X \times A \times X$ and $\pi_1$ any. \label{alg2: line1}
				\State $\pi_1 \gets$ select any policy
				\For{$t\in[T]$}
				\State Choose policy $\pi_t$ in Algorithm~\ref{alg: Learner-Environment Interaction} and observe feedback from interaction
				% \State Observe trajectory from Algorithm~\ref{alg: Learner-Environment Interaction} \label{alg2: line4}
				% \State Update counters $N_t(x_k,a_k) = N_t(x_k,a_k)+1$ and $M_t(x_{k+1}|x_k,a_k) = M_t(x_{k+1}|x_k,a_k)+1$\label{alg2: line5}
				\State Compute $\mathcal{P}_t$, $\overline{r}_t$, and $\underline{G}_{t} $ \label{alg2: line6}
				%				\State $\underline{G}_{t,i}(x,a) = \widehat{g}_{t,i}(x,a) - \xi_t(x,a)$ , for all $(x,a)\in X \times A,i \in [m]$ \label{alg2: line7}
				%				\State $\overline{r}_{t}(x,a)= \widehat{r}_{t}(x,a) + \phi_t(x,a)$, for all  $(x,a)\in X \times A$ \label{alg2: line8}
				\State $q \gets $ solution to  $\text{\texttt{OPT-CB}}_{\Delta(\mathcal{P}_t),\overline{r}_t,\underline{G}_t, {\alpha}}$
				\If{problem is \emph{feasible}} \label{alg2: line9}
				\State $\widehat{q}_{t+1} \gets q$ \label{alg2: line10}
				\Else 
				\State $\widehat q_{t+1} \gets $ take any $q\in\Delta(\mathcal{P}_t)$ \label{alg2: line12}
				\EndIf
				\State $\pi_{t+1} \gets \pi^{\widehat{q}_{t+1}}$ \label{alg2: line13}
				\EndFor
			\end{algorithmic}
		\end{algorithm}


Algorithm~\ref{alg:NS_UCSPS} selects policies with an UCB-like approach encompassing \emph{optimism} in both rewards and constraints satisfaction, following an approach similar to that employed by~\citet{Exploration_Exploitation}.
%
Specifically, at each episode $t \in [T]$ and for any  state-action pair $(x,a) \in X \times A$, the algorithm employs an \emph{upper} confidence bound for the reward $r_t(x,a)$, defined as $\overline r_t(x,a) \coloneqq \widehat{r}_{t}(x,a) + \phi_t(x,a)$, while it uses \emph{lower} confidence bounds for the constraint costs $g_{t,i}(x,a)$, defined as $\underline{g}_{t,i}(x,a) \coloneqq \widehat{g}_{t,i}(x,a) - \xi_t(x,a)$ for every constraint $i \in [m]$.
%
Then, by letting $\overline r_t \in [0,1]^{|X \times A|}$ be the vector with components $\overline r_t(x,a)$ and $\underline{G}_t$ be the matrix with entries $\underline{g}_{t,i}(x,a)$, Algorithm~\ref{alg:NS_UCSPS} chooses the policy to be employed in the next episode $t+1$ by solving the following linear program:
%
\begin{equation}\label{lp:opt_opt}
	\text{\texttt{OPT-CB}}_{\Delta(\mathcal{P}_t), \overline r_t, \underline{G}_t, \alpha} \coloneqq \begin{cases}
		\argmax_{  q \in \Delta(\mathcal{P}_t)} &   \overline r_t^{\top}  q \quad \text{s.t.}\\
	& \underline G_t^{\top}  q \leq  {\alpha},
	\end{cases}
\end{equation}
where $\Delta(\mathcal{P}_t)$ is the set of all the possible valid occupancy measures given the confidence set $\mathcal{P}_t$ (see Appendix~\ref{app:auxiliary}).
%
%Notice that, due to the optimistic nature of Program~\eqref{lp:opt_opt}, both with respect to the non-stationarity and with respect to the parameter estimation, it is possible to show that $\text{\texttt{OPT}}_{\Delta(\mathcal{P}_t), \overline r_t, \underline{G}_t, \underline{\alpha}}$ admits a solution with high probability, and, precisely, its decision space contains the optimum $q^*$ with the same probability.
%
If $\texttt{OPT-CB}_{\Delta(\mathcal{P}_t), \overline r_t, \underline{G}_t, \alpha}$ is feasible, its solution is used to compute a policy to be employed in the next episode, otherwise the algorithm uses any occupancy measure in the set $\Delta(\mathcal P_t)$.
%
% Finally, the policy associated to the chosen occupancy is picked (Line~\ref{alg2: line13}).








\begin{comment}

In Algorithm~\ref{alg:NS_UCSPS} we provide the pseudocode \texttt{NS-UCSPS}.
Precisely, the algorithm initializes the counters to zero, while the confidence interval are initialized to the maximum, that is, one. Furthermore, the algorithm initializes the policy randomly (Line~\ref{alg2: line1}). For any episode, the algorithm plays the policy $\pi_t$ and observes the sample of the rewards and constraints cost associated to the path traversed by the learner (see Line~\ref{alg2: line4}). Once the feedback is received, the counters and the confidence sets are updated accordingly (Lines~\ref{alg2: line5}-\ref{alg2: line6}). Thus, the algorithm builds an optimistic estimate of both the reward and the constraint costs, that is, an upper bound, with high probability, to the reward function (Line~\ref{alg2: line7}) and a lower bound, with high probability, to the constraint costs (Line~\ref{alg2: line8}). The policy for the next episode is chosen by means of the following optimistic linear program:
\begin{equation}
	\label{lp:opt_opt}\text{\texttt{OPT}}_{\Delta(\mathcal{P}_t), \overline r_t, \underline{G}_t, \underline{\alpha}}:=\begin{cases}
		\argmax_{  q \in \Delta(\mathcal{P}_t)} &   \overline r_t^{\top}  q\\
		s.t. & \underline G_t^{\top}  q \leq  \underline{\alpha} 
	\end{cases},
\end{equation}
where $\Delta(\mathcal{P}_t)$ is the set of any possible valid occupancy measure built given $\mathcal{P}_t$ (see Appendix~\ref{app:auxiliary} for the complete definition).
Notice that, due to the optimistic nature of Program~\eqref{lp:opt_opt}, both with respect to the non-stationarity and with respect to the parameter estimation, it is possible to show that $\text{\texttt{OPT}}_{\Delta(\mathcal{P}_t), \overline r_t, \underline{G}_t, \underline{\alpha}}$ admits a solution with high probability, and, precisely, its decision space contains the optimum $q^*$ with the same probability.
 Thus, in case Program~\eqref{lp:opt_opt} admits a feasible solution (see Line~\ref{alg2: line9}), the solution to the aforementioned LP is chosen (Line~\ref{alg2: line10}), otherwise a random occupancy in $\Delta(\mathcal P_t)$ is selected (Line~\ref{alg2: line12}). Finally, the policy associated to the chosen occupancy is picked (Line~\ref{alg2: line13}).

\end{comment}


\subsection{Theoretical guarantees of \texttt{NS-SOPS}}

Next, we prove the theoretical guarantees attained by Algorithm~\ref{alg:NS_UCSPS} (see Appendix~\ref{app:known_c} for complete proofs of the theorems and associated lemmas).
%
First, we analyze the positive cumulative violation incurred by the algorithm.
%
Formally, we can state the following result.
%
%; precisely, it is possible to state the following result:
\begin{restatable}{theorem}{violationbound}\label{theo: violationbound}
	Given any $\delta\in(0,1)$, with probability at least $1-8\delta$, Algorithm~\ref{alg:NS_UCSPS} attains:
	\begin{equation*}
		V_T = \mathcal{O}\left(L|X||A|\sqrt{T\ln\left(\nicefrac{mT|X||A|}{\delta}\right)}+\ln(T)|X||A|C\right).
	\end{equation*}
\end{restatable}
%
Intuitively, Theorem~\ref{theo: violationbound} is proved by showing that every constraint-satisfying occupancy measure is also feasible for Program~\eqref{lp:opt_opt} with high probability.
%
This holds since Program~\eqref{lp:opt_opt} employs lower confidence bounds for constraint costs.
%
Thus, in order to bound $V_T$, it is sufficient to analyze at which rate the feasible region of Program~\eqref{lp:opt_opt} concentrates to the \emph{true} one (\emph{i.e.}, the one defined by $\overline{G}$ in Program~\eqref{lp:offline_opt}).
%
Since by definition of $\xi_t(x,a)$ the feasibility region of Program~\eqref{lp:opt_opt} concentrates as $1/\sqrt{t}+C/t$, the resulting bound for the positive constraint violation $V_T$ is of the order of $\tilde{\mathcal{O}}(\sqrt{T}+C)$.

The regret guaranteed by Algorithm~\ref{alg:NS_UCSPS} is formalized by the following theorem.
%
\begin{restatable}{theorem}{regretknownCG}\label{theo:regretknownCG}
	Given any $\delta \in (0,1)$, with probability at least $1-9\delta$, Algorithm~\ref{alg:NS_UCSPS} attains:
	\begin{equation*}
		R_T= \mathcal{O}\left( L|X||A|\sqrt{T \ln \left(\nicefrac{T|X||A|}{\delta}\right)}+ \ln(T)|X||A|C\right).
	\end{equation*}
\end{restatable}
%
Theorem~\ref{theo:regretknownCG} is proved similarly to Theorem~\ref{theo: violationbound}.
%
Indeed, since every constraint-satisfying occupancy measure is feasible for Program~\eqref{lp:opt_opt} with high probability, this also holds for $q^*$, as it satisfies constraints by definition.
%
Thus, since by definition of $\phi_t(x,a)$ the upper confidence bound for the rewards maximized by Program~\eqref{lp:opt_opt} concentrates as $1/\sqrt{t}+C/t$, the regret bound follows.



\begin{remark}[What if some under/overestimate of $C$ is available]
	%
	We also study what happens if the learner runs Algorithm~\ref{alg:NS_UCSPS} with an under/overestimate on the adversarial corruption as input.
	%
	We defer to Appendix~\ref{app:C_notprecise} all the technical results related to this analysis.
	%
	In particular, it is possible to show that any underestimate on $C$ does not detriment the bound on $V_T$, which remains the one in Theorem~\ref{theo: violationbound}.
	%
	On the other hand, an overestimate on $C$, say $\widehat{C}>C$, results in a bound on $V_T$ of the order of $\mathcal{O}(\sqrt T + \widehat{C})$, which is worse than the one in Theorem~\ref{theo: violationbound}.
	%
	Intuitively, this is because using an overestimate makes Algorithm~\ref{alg:NS_UCSPS} too conservative.
	%
	As a result, one could be tempted to conclude that running Algorithm~\ref{alg:NS_UCSPS} with an underestimate of $C$ as input is satisfactory when the true value of $C$ is unknown.
	%
	However, this would lead to a regret $R_T$ growing linearly in $T$, since, intuitively, a regret-minimizing policy could be cut off from the algorithm decision space.
	%
	This motivates the introduction of additional tools to deal with the case in which $C$ is unknown, as we do in Section~\ref{sec: unknown_C}. 
	%	
	%	It is of interest to study the violation bound of Algorithm~\ref{alg:NS_UCSPS} when it is given as input a guess on the corruption, namely, both an overestimate and an underestimate of the true corruption value. Precisely, it is possible to show that any underestimate of the constraint corruption does not damage the violation bound, that is, the same result as in Theorem~\ref{theo: violationbound} is attained. Differently, given a $\widehat{C}>C$ as input, that is, an overestimate of the corruption, the bound is of order $\mathcal{O}(\sqrt T + \widehat{C})$, thus worsening the bound. This is reasonable, since, with an overestimate of the corruption, the algorithm is too conservative to achieve the optimal bound. For the associated lemmas we refer to Appendix~\ref{app:C_notprecise}.
	%	%
	%	It is important to notice that, given an underestimate of the constraints corruption, we cannot avoid linear regret, since, in principle, the optimal solution could lie in the decision space which is cut out by the underestimate of $C$. This consideration pushed us to resort to different techniques in order to relax the assumption on the corruption knowledge. This is done in Section~\ref{sec: unknown_C}.
\end{remark}


==> Arxiv/c_unknown.tex <==
\section{Learning when $C$ is \emph{not} known: A Lagrangified meta-procedure}\label{sec: unknown_C}



In this section, we go beyond Section~\ref{sec: known_c} by studying the more relevant case in which the learner does \emph{not} know the value of the adversarial corruption $C$.
%
In order to tackle this challenging scenario, we develop a \emph{meta-procedure} (called \texttt{Lag-FTRL}, see Algorithm~\ref{alg:unknown_c}) that instantiates multiple instances of an algorithm working for the case in which $C$ is known, with each instance taking care of a different ``guess'' on the value of $C$.
%
The \texttt{Lag-FTRL} algorithm is inspired by the work of~\citet{corralling} in the context of classical (unconstrained) multi-armed bandit problems.
%
Let us remark that \texttt{Lag-FTRL} is a general algorithm that is \emph{not} specifically tailored for our non-stationary CMDP setting.
%
Indeed, it could be applied to any non-stationary online learning problem with constraints when the adversarial corruption $C$ is unknown, provided that an algorithm working for known $C$ is available.
%
In this section, to deal with our non-stationary CMDP setting, we let \texttt{Lag-FTRL} instantiate multiple instances of the \texttt{NS-SOPS} algorithm developed in Section~\ref{sec: known_c}.
%
%In practice, having a good estimate of the true corruption value $C$ before interacting with the environment is a very strong limitation. In this section, inspired by the work of~\citet{corralling} on unconstrained MAB, we manage to relax the aforementioned assumption, developing a master algorithm which employs different instances of Algorithm~\ref{alg:UOB-REPS with known $C^G$} in order to attain similar regret and violations guarantees.



\subsection{\texttt{Lag-FTRL}: Lagrangified FTRL}






At a high level, the \emph{Lagrangified follow-the-regularized-leader} (\texttt{Lag-FTRL} for short) algorithm works by instantiating several different instances of Algorithm~\ref{alg:NS_UCSPS}, with each instance $\texttt{Alg}^j$ being run for a different ``guess'' of the (unknown) adversarial corruption value $C$.
%
The algorithm plays the role of a \emph{master} by choosing which instance $\texttt{Alg}^j$ to use at each episode.
%
The selection is done by employing an FTRL approach with a suitable log-barrier regularization.
%
In particular, at each episode $t \in [T]$, by letting $\texttt{Alg}^{j_t}$ be the selected instance, the \texttt{Lag-FTRL} algorithm employs the policy $\pi_t^{j_i}$ prescribed by $\texttt{Alg}^{j_t}$ and provides the observed feedback to instance $\texttt{Alg}^{j_t}$ only.


The \texttt{Lag-FTRL} algorithm faces two main challenges.
%
First, the feedback available to the FTRL procedure implemented at the master level is \emph{partial}.
%
This is because, at each episode $t \in [T]$, the algorithm only observes the result of using the policy $\pi_t^{j_i}$ prescribed by the chosen instance $\texttt{Alg}^{j_t}$, and \emph{not} those of the policies suggested by other instances.
%
The algorithm tackles this challenge by employing \emph{optimistic loss estimators} in the FTRL selection procedure, following an approach originally introduced by~\citet{neu}.
%
The second challenge originates from the fact that the goal of the algorithm is to keep under control both the regret and the positive constraint violation.
%
This is accomplished by feeding the FTRL procedure with losses constructed starting from the Lagrangian of the offline optimization problem in Program~\eqref{lp:offline_opt}, and suitably modified to manage \emph{positive} violations.
%
%In Algorithm~\ref{alg:unknown_c}, we present the pseudocode of \texttt{Lag-FTRL}, a master algorithm based on an optimistic estimate of the Lagrangian CMDP formulation with positive constraint violation and on a FTRL with log-barrier kind of update. At high-level, Algorithm~\ref{alg:unknown_c} aims at optimizing over different instances of Algorithm~\ref{alg:NS_UCSPS}. Indeed, there are two main challenge to face. First of all, the feedback received by the master algorithm is \emph{partial}, that is, only the loss function associated to the instance chosen at episode $t\in[T]$ is revealed. This challenge is tackled employing an optimistic estimator of the loss function (as in~\citet{neu}), which allows us to guarantees high-probability bounds. Secondly, the objective function of the master algorithm has to take into account both the regret and the violations attains by the subroutines. This is done by properly build a Lagrangian-like loss function for any instance of Algorithm~\ref{alg:NS_UCSPS}, which encompasses both the rewards and positive violations attained by that specific subroutine.


		\begin{algorithm}[H]
			%\caption{Lagrangified FTRL with Log-Barrier Regularizer}
			\caption{\texttt{Lag-FTRL}}
			\label{alg:unknown_c}
			\begin{algorithmic}[1]
				% \Require $X,A,T,\Lambda=\frac{Lm+1}{\rho},M= \lceil \log_2 T \rceil, \eta= \sqrt{\frac{\ln(T)}{T}}\frac{1}{2L\Lambda},\gamma=\sqrt{\frac{\ln(M/\delta)}{TM}},\alpha,\delta$
				%
				\Require $\delta \in (0,1)$
				\State $\Lambda \gets \frac{Lm+1}{\rho}$, $M \gets  \lceil \log_2 T \rceil$
				\State $\gamma \gets \sqrt{\nicefrac{\ln(M/\delta)}{TM}}$, $\eta \gets \frac{1}{2Lm\Lambda} \sqrt{\nicefrac{\ln(T)}{T}}$
				%
				% \State Initialize $M$ instances of Algorithm \ref{alg:NS_UCSPS},  and initialize each algorithm of index $j \in [M]$ with corruption value $C_j=2^j$ \label{alg3: line1}
				%
				\For{$j \in [M]$}
				\State $\texttt{Alg}^j \gets $ Algorithm~\ref{alg:NS_UCSPS} with $C = 2^j$\label{alg3: line1}
				\EndFor
				\State $w_{1,j} \gets \nicefrac{1}{M}$ for all $j \in [M]$ \label{alg3: line2}
				\For{$t\in[T]$}
				\State Sample index $j_t \sim w_t$ \label{alg3: line4}
				\State $\pi_t^{j_t} \gets $ policy that $\texttt{Alg}^{j_t}$ would choose\label{alg3: line5}
				%
				% \State Observe trajectory as in Algorithm~\ref{alg: Learner-Environment Interaction} and send feedback only to Algorithm $j_t$ \label{alg3: line6}
				%
				\State Choose policy $\pi_t^{j_t}$ in Algorithm~\ref{alg: Learner-Environment Interaction} and observe feedback from interaction
				\State Let $\texttt{Alg}^{j_t}$ observe received feedback\label{alg3: line6}
				%
				% \State Build loss estimator as: $$\ell_{t,j} = \frac{\mathbb{I}(j_t=j)}{w_{t,j}+ \gamma}\left(\sum_{(x_k^t,a_k^t)}\left(1-r_t(x_k^t,a_k^t)\right)+ \Lambda\sum_{i \in [m]}\left[\widehat{g}_{t,i}^j{}^\top \widehat{q}_t^j - \alpha_i\right]^+\right) , \quad \forall j \in [M] $$\label{alg3: line7}
				%
				\For{$j \in [M]$}
				\State Build $\ell_{t,j}$ as in Equation~\eqref{eq:loss_estimator} \label{alg3: line7}
				\EndFor
				%
				\State $\displaystyle w_{t+1} \gets \argmin_{w \in \Delta_M} \, w^\top \sum_{\tau \in [t]}\ell_t + \frac{1}{\eta}\sum_{j\in[M]} \frac{1}{w_j}$ \label{alg3: line8}
				%
				%\State Update weights as: $$ w_{t+1}= \argmin_{w \in \Delta_M} ~ \left(\sum_{\tau \in [t]}\ell_t\right)^\top w + \frac{1}{\eta}\sum_{j\in[M]} \frac{1}{w_j}$$ \label{alg3: line8}
				\EndFor
			\end{algorithmic}
		\end{algorithm}


The pseudocode of the \texttt{Lag-FTRL} algorithm is provided in Algorithm~\ref{alg:unknown_c}.
%
At Line~\ref{alg3: line1}, it instantiates $M \coloneqq\lceil \log_2 T \rceil$ instances of Algorithm~\ref{alg:NS_UCSPS}, with each instance $\texttt{Alg}^j$, for $j \in [M]$, receiving as input a ``guess'' on the adversarial corruption $C=2^j$.
%
The algorithm assigns weights defining a probability distribution to instances $\texttt{Alg}^j$, with $w_{t,j} \in [0,1]$ denoting the weight of instance $\texttt{Alg}^j$ at episode $t \in [T]$.
%
We denote by $w_t \in\Delta_M$ the weight vector at episode $t $, with $\Delta_M$ being the $M$-dimensional simplex.
%
At the first episode, all the weights $w_{1,j}$ are initialized to the value $\nicefrac{1}{M}$ (Line~\ref{alg3: line2}).
%
Then, at each episode $t\in[T]$, the algorithm samples an instance index $j_t \in [M]$ according to the probability distribution defined by the weight vector $w_t$ (Line~\ref{alg3: line4}), and it employs the policy $\pi_t^{j_t}$ prescribed by $\texttt{Alg}^{j_t}$ (Line~\ref{alg3: line5}).
%
The algorithm observes the feedback from the interaction described in Algorithm~\ref{alg: Learner-Environment Interaction} and it sends such a feedback to instance $\texttt{Alg}^{j_t}$ (Line~\ref{alg3: line6}).
%
Then, at Line~\ref{alg3: line7}, the algorithm builds an \emph{optimistic} loss estimator to be fed into each instance $\texttt{Alg}^j$.
%
In particular, at episode $t \in [T]$ and for every $j\in[M]$, the optimistic loss estimator is defined as:
\begin{equation}\label{eq:loss_estimator}
	\ell_{t,j} \coloneqq \frac{\mathbb{I}(j_t=j)}{w_{t,j}+ \gamma}\Bigg( L - \sum_{k \in [0 \ldots L-1]}r_t(x_k^t,a_k^t)+ \Lambda\sum_{i \in [m]}\left[ \Big( \widehat{G}_{t}^{j} \Big)^\top \, \widehat{q}_t^j - \alpha\right]_i^+\Bigg),
\end{equation}
where $\gamma$ is a suitably-defined implicit exploration factor, $(x_k^t,a_k^t)$ is the state-action pair visited at layer $k$ during episode $t $, $\Lambda$ is a suitably-defined upper bound on the optimal values of Lagrangian multipliers,\footnote{Notice that, in the definition of $\Lambda$, $\rho$ is the feasibility parameter of Program~\eqref{lp:offline_opt} for the reward vector $\overline{r}$, the constraint cost matrix $\overline{G}$, and the threshold vector $\alpha$. In order to compute $\Lambda$, Algorithm~\ref{alg:unknown_c} needs knowledge of $\rho$. Nevertheless, our results continue to hold even if Algorithm~\ref{alg:unknown_c} is only given access to a lower bound on $\rho$.} $\widehat{G}_{t}^j$ is the matrix of empirical constraint costs built by the instance $\texttt{Alg}^j$ of Algorithm~\ref{alg:NS_UCSPS} at episode $t$, while $\widehat q_t^j$ is the occupancy measure computed by instance $\texttt{Alg}^j$ of Algorithm~\ref{alg:NS_UCSPS} at $t$.
%
Finally, the algorithm updates the weight vector according to an FTRL update with a suitable log-barrier regularization (see Line~\ref{alg3: line8} for the definition of the update).



\subsection{Theoretical guarantees of \texttt{Lag-FTRL}}

Next, we prove the theoretical guarantees attained by Algorithm~\ref{alg:unknown_c} (see Appendix~\ref{app:unknown_C} for complete proofs of the theorems and associated lemmas).
%
As a first preliminary step, we extend the well-known strong duality result for CMDPs~\citep{Altman1999ConstrainedMD} to the case of bounded Lagrangian multipliers.
%
\begin{restatable}{lemma}{strongDuality}\label{lemma:auxiliary dual}
	Given a CMDP with a transition function $P$, for every reward vector $r \in [0,1]^{|X \times A|}$, constraint cost matrix $G \in [0,1]^{|X \times A| \times m}$, and threshold vector $\alpha \in [0,L]^m$, if Program~\eqref{lp:offline_opt} satisfies Slater's condition (Condition~\ref{cond:slater}), then the following holds:
	%
	% Given a reward vector $r$, a cost matrix $G$ and the thresholds vector $\alpha$, if Slater's condition holds with parameter $\rho$ for Program~\eqref{lp:offline_opt}, for $\lambda\in\mathbb{R}^m_{\geq0}$, it holds:
	%
	\begin{align*}
		\min_{\lVert \lambda \rVert_1\in [0,\nicefrac{L}{\rho}]} \max_{  q \in \Delta(P)} r^\top q - \sum_{i \in [m]}\lambda_i\left[ {G}^\top q-\alpha \right]_i & =   \max_{  q \in \Delta(P)} \min_{\lVert \lambda \rVert_1\in [0,\nicefrac{L}{\rho}]}r^\top q - \sum_{i \in [m]}\lambda_i \left[ {G}^\top q-\alpha \right]_i  \\&= \textnormal{OPT}_{r,G,\alpha},
	\end{align*}
	%
	where $\lambda\in\mathbb{R}^m_{\geq0}$ is a vector of Lagrangian multipliers and $\rho$ is the feasibility parameter of Program~\eqref{lp:offline_opt}.
	%
\end{restatable}
%
Intuitively, Lemma~\ref{lemma:auxiliary dual} states that, under Slater's condition, strong duality continues to hold even when restricting the set of Lagrangian multipliers to the $\lambda\in\mathbb{R}^m_{\geq0}$ having $\lVert \lambda \rVert_1$ bounded by $\nicefrac{L}{\rho}$. 
%
Furthermore, we extend the result in Lemma~\ref{lemma:auxiliary dual} to the case of a Lagrangian function suitably-modified to encompass \emph{positive} violations.
%
We call it \emph{positive Lagrangian} of Program~\eqref{lp:offline_opt}, defined as follows.
%
\begin{definition}[Positive Lagrangian]
	Given a CMDP with a transition function $P$, for every reward vector $r \in [0,1]^{|X \times A|}$, constraint cost matrix $G \in [0,1]^{|X \times A| \times m}$, and threshold vector $\alpha \in [0,L]^m$, the \emph{positive Lagrangian} of Program~\eqref{lp:offline_opt} is defined as a function $\mathcal{L} : \mathbb{R}_+ \times \Delta(P) \to \mathbb{R}$ such that it holds $\mathcal{L}\left(\beta,q\right) \coloneqq r^\top q - \beta \sum_{i \in [m]}\left[{G}^\top q-\alpha\right]_i^+$ for every $\beta \geq 0$ and $q\in \Delta(P).$
	%
	%	Given a reward vector $r$, a cost matrix $G$ and the thresholds vector $\alpha$, we define the positive Lagrangian function for Program~\eqref{lp:offline_opt} as
	%		$\mathcal{L}\left(\Sigma,q\right)= r^\top q - \Sigma\sum_{i \in [m]}\left[{G}_{i}^\top q-\alpha_i\right]^+.$
\end{definition}
%
The positive Lagrangian is related to the Lagrangian of a variation of Program~\eqref{lp:offline_opt} in which the $[\cdot]^+$ operator is applied to the constraints.
%
Notice that such a problem does \emph{not} admit Slater's condition, since, by definition of $[\cdot]^+$, it does \emph{not} exist an occupancy measure $q^\circ$ such that $\left[{G}^\top q^\circ-\alpha\right]_i^+ < 0$ for every $i\in[m]$.
%
Nevertheless, we show that a kind of strong duality result still holds for $\mathcal{L}(\nicefrac{L}{\rho},q)$, when Slater's condition is met by Program~\eqref{lp:offline_opt}. This is done in the following result.
%
% the offline optimization problem defining the positive Lagrangian does \emph{not} admit Slater's condition, since, by definition of the $[\cdot]^+$ operator, it does not exist an occupancy measure such that $q^\circ$ s.t. $\left[{G}^\top q^\circ-\alpha\right]_i^+\leq 0$ for any $i\in[m]$. Nevertheless, we show that a strong duality-kind of result still holds for $\mathcal{L}(\nicefrac{L}{\rho},q)$, when Slater's condition holds for the optimization problem when the $[\cdot]^+$ operator is not applied to the constraints, namely, Program~\eqref{lp:offline_opt}. This is done in the following result.
%
% Thus, we are ready to extend the previous result to the positive Lagrangian.
%
\begin{restatable}{theorem}{positiveStrongDuality}\label{theo: strong duality}
		Given a CMDP with a transition function $P$, for every reward vector $r \in [0,1]^{|X \times A|}$, constraint cost matrix $G \in [0,1]^{|X \times A| \times m}$, and threshold vector $\alpha \in [0,L]^m$, if Program~\eqref{lp:offline_opt} satisfies Slater's condition (Condition~\ref{cond:slater}), then the following holds:
		%
		% Given a reward vector $r$, a cost matrix $G$ and the thresholds vector $\alpha$, if Slater's condition holds with parameter $\rho$ for Program~\eqref{lp:offline_opt}, it holds:
		%
		\begin{align*}
			\max_{q \in \Delta(P)}\mathcal{L}(\nicefrac L \rho,q) = \max_{q \in \Delta(P)} r^\top q - \frac{L}{\rho}\sum_{i \in [m]}\left[{G}^\top q-\alpha \right]_i^+  = \textnormal{OPT}_{r,G,\alpha},
		\end{align*}
		%
		where $\rho$ is the feasibility parameter of Program~\eqref{lp:offline_opt}.
\end{restatable}
%
Theorem~\ref{theo: strong duality} intuitively shows that a $L/\rho$ multiplicative factor on the positive constraint violation is enough to compensate the large rewards that non-feasible policies would attain when employed by the learner. 
%
This result is crucial since, without properly defining the Lagrangian function optimized by Algorithm~\ref{alg:unknown_c}, the FTRL optimization procedure would choose instances with both large rewards and large constraint violation, thus preventing the violation bound from being sublinear.

By means of Theorem~\ref{theo: strong duality}, it is possible to provide the following result.
%
\begin{restatable}{theorem}{ViolationUnknown}
	\label{theo:ViolationUnknown}
	If Program~\eqref{lp:offline_opt} instantiated with $\overline{r}$, $\overline{G}$ and $\alpha$ satisfies Slater's condition (Condition~\ref{cond:slater}), then, given any $\delta \in (0,1)$, Algorithm \ref{alg:unknown_c} attains the following bound with probability at least $1-30\delta$:
	\begin{equation*}
		V_T= \mathcal{O}\left(m^2L^2|X||A|\sqrt{T\ln\left(\nicefrac{mT|X||A|}{\delta}\right)}\ln(T)+ m^2L\ln(T)|X||A|C\right).
	\end{equation*}
\end{restatable}
%
Intuitively, to prove Theorem~\ref{theo:ViolationUnknown}, it is necessary to bound the negative regret attained by the algorithm, \emph{i.e.}, how better Algorithm~\ref{alg:unknown_c} can perform in terms of rewards with respect to an optimal occupancy in hindsight $q^*$. Notice that this is equivalent to showing that the FTRL procedure cannot gain more than $\textnormal{OPT}_{\overline r,\overline G,\alpha}$ by playing policies that are \emph{not} feasible, or, equivalently, by choosing instances $\texttt{Alg}^j$ with a large corruption guess, which, by definition of the confidence sets employed by Algorithm~\ref{alg:NS_UCSPS}, may play non-feasible policies attaining large rewards.
%
This is done by employing Theorem~\ref{theo: strong duality}, which shows that the positive Lagrangian does \emph{not} allow the algorithm to achieve too large rewards with respect to $q^*$.
%
Thus, the violations are still upper bounded by $\tilde{\mathcal{O}} (\sqrt{T}+C)$.

Finally, we prove the regret bound attained by Algorithm~\ref{alg:unknown_c}.
%
\begin{restatable}{theorem}{RegretUnknown}\label{Theo:RegretUnknown}
	If Program~\eqref{lp:offline_opt} instantiated with $\overline{r}$, $\overline{G}$ and $\alpha$ satisfies Slater's condition (Condition~\ref{cond:slater}), then, given any $\delta \in (0,1)$, Algorithm \ref{alg:unknown_c} attains the following bound with probability at least $1-26\delta$:
	\begin{equation*}
		R_T  = \mathcal{O}\left(m^2L^2|X||A|\sqrt{T\ln\left(\nicefrac{mT|X||A|}{\delta}\right)}\ln(T)+ m^2L\ln(T)|X||A|C\right).
	\end{equation*}
\end{restatable}
%
Bounding the regret attained by Algorithm~\ref{alg:unknown_c} requires different techniques with respect to bounding constraint violation. Indeed, strong duality is \emph{not} needed, since, even if $\Lambda$ is set to a too small value and thus the algorithm plays non-feasible policies, then the regret would still be sublinear. 
The regret bound is strongly related to the optimal value of the problem associated with the positive Lagrangian, which, by definition of $[\cdot]^+$ cannot perform worse than the optimum of Program~\eqref{lp:offline_opt}, in terms of rewards gained.
%
Thus, by letting $j^*$ be the index of the instance associated with true corruption value $C$, proving Theorem~\ref{Theo:RegretUnknown} reduces to bounding the regret and the constraint violation of instance $\texttt{Alg}^{j^*}$, with the additional challenge of bounding the estimation error of the optimistic loss estimator. Finally, by means of the results for the \emph{known} $C$ case derived in Section~\ref{sec: known_c}, we are able to show that the regret is at most $\tilde{\mathcal{O}} (\sqrt{T}+C)$, which is the desired bound.

==> Arxiv/introduction.tex <==
\section{Introduction}\label{introduction}

Reinforcement learning~\citep{sutton2018reinforcement} is concerned with settings where a learner sequentially interacts with an environment modeled as a \emph{Markov decision process} (MDP)~\citep{puterman2014markov}.
%
Most of the works in the field focus on learning policies that maximize learner's rewards.
%
However, in most of the real-world applications of interest, the learner also has to meet some additional requirements.
%
For instance, autonomous vehicles must avoid crashing~\citep{isele2018safe,wen2020safe}, bidding agents in ad auctions must \emph{not} deplete their budget~\citep{wu2018budget,he2021unified}, and users of recommender systems must \emph{not} be exposed to offending content~\citep{singh2020building}.
%
These requirements can be captured by \emph{constrained} MDPs (CMDPs)~\citep{Altman1999ConstrainedMD}, which generalize MDPs by specifying constraints that the learner has to satisfy while maximizing their rewards.


We study \emph{online learning} in \emph{episodic} CMDPs~(see, \emph{e.g.},~\citep{Exploration_Exploitation}), where the goal of the learner is twofold.
%
On the one hand, the learner wants to minimize their \emph{regret}, which measures how much reward they lost over the episodes compared to what they would have obtained by always using a best-in-hindsight constraint-satisfying policy.
%
On the other hand, the learner wants to ensure that the \emph{(cumulative) constraint violation} is minimized during the learning process.
%
Ideally, one seeks for algorithms with both regret and constraint violation growing sublinearly in the number of episodes $T$.


A crucial feature distinguishing online learning problems in CMDPs is whether rewards and constraints are selected \emph{stochastically} or \emph{adversarially}.
%
Most of the works focus on the case in which constraints are stochastic (see, \emph{e.g.},~\citep{Online_Learning_in_Weakly_Coupled,Constrained_Upper_Confidence,Exploration_Exploitation,Upper_Confidence_Primal_Dual,bounded,bai2023}), with only one exception addressing settings with adversarial constraints~\citep{germano2023bestofbothworlds}.
%
This is primarily motivated by a well-known impossibility result by~\citet{Mannor}, which prevents any learning algorithm from attaining both sublinear regret and sublinear constraint violation, when competing against a best-in-hindsight policy that satisfies the constraints \emph{on average}.
%
However, dealing with adversarially-selected constraints is of paramount importance to cope with real-world environments, which are typically non-stationary.
%
% Indeed, in most of the real-world applications, constraints change over the episodes.
%
% it is unreasonable to assume that constraints are selected stochastically according to a fixed probability distribution, as they rather change over the episodes.

% \albo{Mi sa che le cit ho messe a cazzo perchè mi confondono i nomi delle references.}


\subsection{Original contributions}

The main contribution of this paper is to show how to ease the negative result of~\citep{Mannor}, by considering CMDPs with \emph{non-stationary rewards and constraints}.
%
Specifically, we address CMDPs where rewards and constraints are selected from probability distributions that are allowed to change \emph{adversarially} from episode to episode.
%
One may think of our setting as bridging the gap between fully-stochastic and fully-adversarial ones.
%
We design algorithms whose performances---in terms of regret and constraint violation---smoothly degrade as a suitable measure of non-stationarity increases.
%
This is called \emph{(adversarial) corruption}, as it intuitively quantifies how much the distributions of rewards and constraints vary over the episodes with respect to some ``fictitious'' non-corrupted counterparts.


We propose algorithms that attain $\tilde{\mathcal{O}} (\sqrt{T} + C)$ regret and constraint violation, where $C$ denotes the corruption of the setting.
%
We remark that $C$ can be $\Theta(T)$ in the worst case, and, thus, our bounds are coherent with the impossibility result by~\citet{Mannor}.
%
Notably, our algorithms work under \emph{bandit} feedback, namely, by only observing rewards and constraint costs of the state-action pairs visiting during episodes.
%
Moreover, they are able to manage \emph{positive} constraint violation.
%
This means that they do \emph{not} allow for a negative violation (\emph{i.e.}, a constraint satisfaction) to cancel out a positive one across different episodes.
%
This is a crucial requirement for most of the practical applications.
%
For instance, in autonomous driving, avoiding a collision does \emph{not} ``repair'' a previously-occurred crash.



In the first part of the paper, we design an algorithm, called \texttt{NS-SOPS}, which works assuming that the value of the corruption $C$ is known.
%
This algorithm achieves $\tilde{\mathcal{O}} (\sqrt{T} + C)$ regret and positive constraint violation by employing a \emph{policy search} method that is \emph{optimistic} in both reward maximization and constraint satisfaction.
%
Specifically, the algorithm incorporates $C$ in the confidence bounds of rewards and constraint costs, so as to ``boost'' its optimism and achieve the desired guarantees.


In the second part of the paper, we show how to embed the \texttt{NS-SOPS} algorithm in a \emph{meta-procedure} that allows to achieve $\tilde{\mathcal{O}} (\sqrt{T} + C)$ regret and positive constraint violation when $C$ is \emph{unknown}.
%
The meta-procedure works by instantiating multiple instances of an algorithm for the case in which $C$ is known, each one taking care of a different ``guess'' on the value of $C$.
%
Specifically, the meta-procedure acts as a \emph{master} by choosing which instance to follow in order to select a policy at each episode.
%
To do so, it employs an adversarial online learning algorithm, which is fed with losses constructed starting from the Lagrangian of the CMDP problem, suitably modified to account for \emph{positive} constraint violation.
%
%it employs an FTRL approach with a suitable log-barrier regularization, fed with losses constructed starting from the Lagrangian of the CMDP problem, suitably modified to account for positive constraint violations.
%
Our meta-procedure is of independent interest, as it can be applied in \emph{any} non-stationary constrained online learning setting, so as to relax the knowledge of $C$.


\subsection{Related works}



Within the literature on CMDPs, settings with \emph{stochastic} rewards and constraints have been widely investigated.
%
However, their \emph{non-stationary} counterparts, including \emph{adversarial} ones in the worst case, are still largely unexplored.
%
In the following, we discuss the works that are most related to ours, while we refer the reader to Appendix~\ref{app:related} for a comprehensive survey of related works.
%
% In the following, we highlight the works which are most related to ours. Due to space constraints, we refer to Appendix~\ref{app:related} for a complete discussion on related works. While online learning in CMDPs with stochastic rewards and constraints have been widely studied (see, \emph{e.g.},~\citep{Exploration_Exploitation}), the non-stationary (in worst case adversarial) counterpart is far to be completely explored. Specifically, the following are the main works that deal with online CMDPs in presence of non-stationarity. 

%\stradi{questa frase vogliamo leggermente riformularla per renderla meno aggressiva?}

\citet{Upper_Confidence_Primal_Dual} provide the first primal-dual approach to deal with episodic CMDPs with adversarial losses and stochastic constraints, achieving, under full feedback, both sublinear regret and sublinear (non-positive) constraint violation (\emph{i.e.}, allowing for cancellations). 
%
\citet{stradi2024learning} are the first to tackle CMDPs with adversarial losses and stochastic constraints under {bandit} feedback, by proposing an algorithm that achieves sublinear regret and sublinear positive constraint violation.
%, assuming that the constraint are stochastic.
%
These works do \emph{not} consider settings where constraints are non-stationary, \emph{i.e.}, they may change over the episodes.

\citet{ding_non_stationary}~and~\citet{wei2023provably} consider the case in which rewards and constraints are non-stationary, assuming that their variation is bounded.
%, as in our work.
%
Our work differs from theirs in multiple aspects.
%
First, we consider \emph{positive} constraint violation, while they allow for cancellations.
%
As concerns the definition of regret, ours and that used by \citet{ding_non_stationary}~and~\citet{wei2023provably} are \emph{not} comparable.
%
Indeed, they employ a dynamic regret baseline, which, in general, is harder than the static regret employed in our work.
%
However, they compare learner's performances against a dynamic policy that satisfies the constraints at every round.
%
Instead, we consider a policy that satisfies the constraints \emph{on average}, which can perform arbitrarily better than a policy satisfying the constraints at every round.
%
Furthermore, the dependence on $T$ in their regret bound is much worse than ours, even when the non-stationarity is small, namely, when it is a constant independent of $T$ (and, thus, dynamic regret collapses to static regret).
%
Finally, we do \emph{not} make any assumption on $T$, while both regret and constraint violation bounds in~\citep{wei2023provably} only hold for large $T$.


Finally,~\citet{germano2023bestofbothworlds} are the first to study CMDPs with adversarial constraints.
%
Given the impossibility result by~\citet{Mannor}, they propose an algorithm that, under full feedback, attains sublinear (non-positive) constraint violation (\emph{i.e.}, with cancellations allowed) and a fraction of the optimal reward, thus resulting in a regret growing linearly in $T$.
%
We show that sublinear regret and sublinear constraint violation can indeed be attained simultaneously if one takes into account the corruption $C$, which can be seen as a measure of how much adversarial the environment is.
%
% Assuming that the adversariality of the problem is bounded by a corruption measure $C$, we manage to show that sublinear regret and sublinear violations can be attained even when the constraints are non-stationary.
%
Moreover, let us remark that our algorithms deal with \emph{positive} constraint violation under \emph{bandit} feedback, and, thus, they are much more general than those in~\citep{germano2023bestofbothworlds}.



\begin{comment}


\stradi{Parlare bene del rapporto corruzione non stationarity}

\stradi{ho diviso in sezioncine ma forse conviene averne una unica per l'introduction, vedi tu albo}

\begin{itemize}
	\item Discorsetto generale su RL
	\item Discorsetto generale su RL con constraints
	\item Dire che in setting non-stazionario c'è ancora molto da studiare
\end{itemize}

\subsection{Original contribution}
...\stradi{importante dire che il nostro è un setting principalmente avversario, perciò le baseline sono quelle avversarie}

\stradi{forse bisognerebbe agganciarlo ai related work}

\begin{itemize}
	\item partire da risultato di impossibilità di Mannor
	\item dire che noi ci mettiamo nel mezzo tra stocastic e avversario (perciò siamo migliori degli altri miei)
	\item e poi paragone con quegli altri di non-stationary
	\item dire che abbiamo bandit feedback e positive violation
	\item poi potremmo azzardarci a dire che la dipendenza da C è ottima, anche se è vero solo rispetto ad una tra regret e violation
	\item dire che il nostro approccio con unknown C è di independent interest
\end{itemize}
\subsection{Related works}

In the following, we highlight the works which are most related to ours. Due to space constraints, we refer to Appendix~\ref{app:related} for a complete discussion on related works. While online learning in CMDPs with stochastic rewards and constraints have been widely studied (e.g., see~\citep{Exploration_Exploitation} for a seminal work in the field), the non-stationary (in worst case, adversarial) counterpart is far to be completely explored. Precisely, to the best of our knowledge, the following are the only works who deal with online CMDPs in presence of non-stationarity. \stradi{questa frase vogliamo leggermente riformularla per renderla meno aggressiva?}

\citet{Upper_Confidence_Primal_Dual} provide the first primal-dual approach to deal with episodic CMDPs with adversarial losses and stochastic constraints, achieving both sublinear regret and constraint violation (with cancellations allowed) with full-information feedback. 
%
\cite{stradi2024learning} is the first work to tackle CMDPs with adversarial losses and bandit feedback. They propose an algorithm which achieves sublinear regret and sublinear positive constraints violations, assuming that the constraints are stochastic.
%
The aforementioned works do not consider settings in which the constraints are non-stationary, that is, the constraints may change during the episodes

\citet{ding_non_stationary}~and~\citet{wei2023provably} consider the case in which rewards and constraints are non-stationary, assuming that their variation is bounded, as in our work. Nevertheless, our settings differ in multiple aspects. First of all, we consider positive constraints violations, while the aforementioned works allow the cancellations in their definition. As concerns the regret definition, ours and the one proposed in \citet{ding_non_stationary}~and~\citet{wei2023provably} are difficult to compare. Indeed, they employ a dynamic baseline which, in general, is harder than the static regret baseline employed in our work. Nevertheless, they compare them self with a dynamic policy which satisfies the constraints at each round. Contrariwise, we consider a policy which satisfies the constraints on average, which can perform arbitrarily better than a policy which satisfies the constraints at each round. Furthermore, the dependence on $T$ in their regret bound is much worse than ours even when the non-stationarity is small,  namely, when it is a constant indipendent on $T$ (and, the dynamic regret collapses to the standard static regret). Finally, we do not make any assumption on the number of episodes, while both the regret and violations bounds presented in~\citet{wei2023provably} hold only for large $T$.


Finally,~\citet{germano2023bestofbothworlds} are the first to study CMDPs with adversarial constraints. Given the well-known impossibility result to learn with adversarial constraints (see, \citep{Mannor}), they propose an algorithm that attains sublinear violation (with cancellations allowed) and a fraction of the optimal reward when the feedback is full. 
%
Assuming that the adversariality of the problem is bounded by a corruption measure $C$, we manage to show that sublinear regret and sublinear violations can be attained even when the constraints are not  stationary. 
Moreover, we underline the our work considers positive violations and bandit feedback, thus being more general with respect to~\citep{germano2023bestofbothworlds}.


\end{comment}


==> Arxiv/prelim.tex <==
\section{Preliminaries}\label{sec:Preliminaries}


\subsection{Constrained Markov decision processes}


We study \emph{episodic constrained} MDPs~\citep{Altman1999ConstrainedMD} (CMDPs), in which a learner interacts with an unknown environment over $T$ episodes, with the goal of maximizing long-term rewards subject to some constraints.
%
% which are defined as follows.
%
% There is a finite number $T$ of episodes, with $t\in[T]$ denoting a specific episode.\footnote{In this paper, we denote by $[a \ldots b]$ the set of all the natural numbers from $a \in \mathbb{N}$ to $b \in \mathbb{N}$ (both included), while $[b] \coloneqq [ 1 \ldots b ]$ is the set of the first $b \in \mathbb{N}$ natural numbers.}
%
$X$ is a finite set of states of the environment, $A$ is a finite set of actions available to the learner in each state, while the environment dynamics is  governed by a transition function $P : X \times A \times X  \to [0, 1]$, with $P (x^{\prime} |x, a)$ denoting the probability of going from state $x \in X$ to $x^{\prime} \in X$ by taking action $a \in A$.\footnote{In this paper, we consider w.l.o.g.~\emph{loop-free} CMDPs. This means that $X$ is partitioned into $L$ layers $X_{0}, \dots, X_{L}$ such that the first and the last layers are singletons, \emph{i.e.}, $X_{0} = \{x_{0}\}$ and $X_{L} = \{x_{L}\}$. Moreover, the loop-free property implies that $P(x^{\prime} |x, a) > 0$ only if $x^\prime \in X_{k+1}$ and $x \in X_k$ for some $k \in [0 \ldots L-1]$. Notice that any episodic CMDP with horizon $L$ that is \emph{not} loop-free can be cast into a loop-free one by suitably duplicating the state space $L$ times, \emph{i.e.}, a state $x$ is mapped to a set of new states $(x, k)$, where $k \in [0 \ldots L]$.}%. We will refer as $k(x)$ to the index of the layer that $x$ belongs to.}
%
% $P : X \times A \times X  \to [0, 1]$ is a transition function, with $P (x^{\prime} |x, a)$ denoting the probability of going from state $x \in X$ to state $x^{\prime} \in X$ by taking action $a \in A$.
%
At each episode $t \in [T]$,\footnote{In this paper, we denote by $[a \ldots b]$ the set of all the natural numbers from $a \in \mathbb{N}$ to $b \in \mathbb{N}$ (both included), while $[b] \coloneqq [ 1 \ldots b ]$ is the set of the first $b \in \mathbb{N}$ natural numbers.} a reward vector $r_{t} \in [0,1]^{|X\times A|}$ is sampled according to a probability distribution $\mathcal{R}_t$, with $r_t(x,a)$ being the reward of taking action $a \in A$ in state $x \in X$ at episode $t$.
%
Moreover, a constraint cost matrix $G_t \in [0,1]^{|X\times A| \times m }$ is sampled according to a probability distribution $\mathcal{G}_t$, with $g_{t,i}(x,a)$ being the cost of constraint $i \in [m]$ when taking action $a \in A$ in state $x \in X$ at episode $t$.
%
We also denote by $g_{t,i} \in [0,1]^{|X\times A|}$ the vector of all the costs $g_{t,i}(x,a)$ associated with constraint $i$ at episode $t$.
% and $g_{t,i}(x,a)$ being the cost of constraint $i$ when taking action $a \in A$ in state $x \in X$ at episode $t$.
%
Each constraint requires that its corresponding expected cost is kept below a given threshold.
%
The thresholds of all the $m$ constraints are encoded in a vector $\alpha\in [0,L]^m$, with $\alpha_i$ denoting the threshold of the $i$-th constraint.
%
%$\{\mathcal{R}_t\}_{t=1}^T$ is a sequence of probability distributions with support in $[0,1]^{|X\times A|}$.
%%
%At each episode $t \in [T]$, a reward vector $r_{t} \in [0,1]^{|X\times A|}$ is sampled according to $\mathcal{R}_t$, with $r_t(x,a)$ being the reward of taking action $a \in A$ in state $x \in X$ at episode $t$.
%%
%$\{\mathcal{G}_t\}_{t=1}^T$ is a sequence of probability distributions with support in $[0,1]^{|X\times A|\times m}$.
%%
%At each episode $t \in [T]$, a constraints cost matrix $G_t \in [0,1]^{|X\times A|\times m}$ is sampled according to $\mathcal{G}_t$, with $g_{t,i} \in [0,1]^{|X\times A|}$ denoting the vector of all the costs associated with constraint $i \in [m]$ at episode $t$ and $g_{t,i}(x,a)$ being the cost of constraint $i$ when taking action $a \in A$ in state $x \in X$ at episode $t$.
%%
%Finally, $\alpha\in [0,L]^m$ is a vector of cost thresholds that characterize the $m$ constraints, where $\alpha_i$ denotes the threshold for the $i$-th constraint.

We consider a setting in which the sequences of probability distributions $\{\mathcal{R}_t\}_{t=1}^T$ and $\{\mathcal{G}_t\}_{t=1}^T$ are selected \emph{adversarially}.
%
Thus, reward vectors $r_t$ and constraint cost matrices $G_t$ are random variables whose distributions are allowed to change arbitrarily from episode to episode.
%
To measure how much such probability distributions change over the episodes, we introduce the notion of \emph{(adversarial) corruption}.
%
In particular, we define the adversarial corruption $C_r$ for the rewards as follows:
%
\begin{equation}\label{def: C^r}
	C_r \coloneqq \min_{r \in[0,1]^{|X\times A|}}\sum_{t\in [T]}\left\lVert \mathbb{E}[r_{t}] - r \right\rVert_1.
\end{equation}
%
Intuitively, the corruption $C_r$ encodes the sum over all episodes of the distances between the means $\mathbb{E}[r_{t}]$ of the adversarial distributions $\mathcal{R}_t$ and a ``fictitious'' non-corrupted reward vector $r$.
%
Notice that a similar notion of corruption has been employed in unconstrained MDPs to measure the non-stationarity of transition probabilities; see~\citep{jin2024no}. 
%
In the following, we let $r^\circ \in[0,1]^{|X\times A|}$ be a reward vector that attains the minimum in the definition of $C_r$.
%
Similarly, we introduce the adversarial corruption $C_G$ for constraint costs, which is defined as follows:
%
\begin{equation}\label{def: C^G}
	C_G \coloneqq {\min_{g \in[0,1]^{|X\times A|}}}\underset{t\in [T]}{\sum}\underset{i \in [m]}{\max}\lVert \mathbb{E}[g_{t,i}] - g \rVert_1.
\end{equation}
%
We let $g^\circ \in [0,1]^{|X\times A|}$ be the constraint cost vector that attains the minimum in the definition of $C_G$.
%
Finally, we introduce the total adversarial corruption $C$, which is defined as $
C \coloneqq \max\{C_G,C_r\}$.\footnote{In the rest of the paper, for ease of presentation, we derive all our results in terms of the total adversarial corruption $C$. We remark that such results can be easily extended to account for $C_r$ and $C_G$ separately.}


		\begin{algorithm}[]
			\caption{Learner-Environment Interaction}
			\label{alg: Learner-Environment Interaction}
			\begin{algorithmic}[1]
				% \For{$t\in[T]$}
				\State $\mathcal{R}_t$ and $\mathcal{G}_t$ are chosen \textit{adversarially}
				%\State $\{g_{t,i}\}_{i=1}^m$ sampled from the stochastic distribution $\mathcal{G}_t$
				\State Choose a policy $\pi_{t}: X \times A  \to [0, 1]$
				\State Observe initial state $x_{0}$
				\For{$k = 0, \ldots,  L-1$}
				\State Play $a_{k} \sim \pi_t(\cdot|x_{k})$
				\State Observe  $r_t(x_k,a_k)$ and $g_{t,i}(x_k,a_k)$ for $i\in[m]$
				% \State Environment evolves to $x_{k+1}\sim P(\cdot|x_{k},a_{k})$
				\State Observe new state $x_{k+1}\sim P(\cdot|x_{k},a_{k})$
				\EndFor
				% \EndFor
			\end{algorithmic}
		\end{algorithm}

Algorithm~\ref{alg: Learner-Environment Interaction} summarizes how the learner interacts with the environment at episode $t \in [T]$.
%
In particular, the learner chooses a \emph{policy} $\pi: X \times A \to [0,1]$ at each episode, defining a probability distribution over actions to be employed in each state.
%
For ease of notation, we denote by $\pi(\cdot|x)$ the probability distribution for a state $x \in X$, with $\pi(a|x)$ being the probability of selecting action $a \in A$.
%
% Algorithm~\ref{alg: Learner-Environment Interaction} depicts the interaction between the learner and the environment in a CMDP.
%
Let us remark that we assume that the learner knows $X$ and $A$, but they do \emph{not} know anything about $P$.
%
Moreover, the \emph{feedback} received by the learner after each episode is \emph{bandit}, as they observe the realizations of rewards and constraint costs only for the state-action pairs $(x_k,a_k)$ actually visited during that episode.



\subsection{Occupancy measures}


Next, we introduce \emph{occupancy measures}, following the notation by~\citep{OnlineStochasticShortest}.
%
Given a transition function $P$ and a policy $\pi$, the occupancy measure $q^{P,\pi} \in [0, 1]^{|X\times A\times X|}$ induced by $P$ and $\pi$ is such that, for every $x \in X_k$, $a \in A$, and $x^{\prime} \in X_{k+1}$ with $k \in [0 \ldots L-1]$:
\begin{equation}
	q^{P,\pi}(x,a,x^{\prime}) \coloneqq \mathbb{P}[x_{k}=x, a_{k}=a,x_{k+1}=x^{\prime}|P,\pi], \label{def:occupancy_measure}
\end{equation}
%
which represents the probability that, under $P$ and $\pi$, the learner reaches state $x$, plays action $a$, and gets to the next state $x^\prime$.
%
Moreover, we also define the following quantities:
\begin{align}
	q^{P,\pi}(x,a) \coloneqq \sum_{x^\prime\in X_{k+1}}q^{P,\pi}(x,a,x^{\prime}) \quad \text{and} \quad
	q^{P,\pi}(x) \coloneqq \sum_{a\in A}q^{P,\pi}(x,a). \label{def:q vector}
\end{align}

The following lemma characterizes when a vector $  q \in [0, 1]^{|X\times A\times X|}$ is a \emph{valid} occupancy measure.
%
\begin{lemma}[\citet{rosenberg19a}]\label{lem:occupancy_rosenberg}
	A vector $  q \in [0, 1]^{|X\times A\times X|}$ is a {valid} occupancy measure of an episodic loop-free CMDP if and only if it satisfies the following conditions:
	\[
	\begin{cases}
		\displaystyle\sum_{x \in X_{k}}\sum_{a\in A}\sum_{x^{\prime} \in X_{k+1}} q(x,a,x^{\prime})=1 & \forall k\in[0\dots L-1]
		\\ 
		\displaystyle\sum_{a\in A}\sum\limits_{x^{\prime} \in X_{k+1}}q(x,a,x^{\prime})=
		\sum_{x^{\prime}\in X_{k-1}} \sum_{a\in A}q(x^{\prime},a,x) & \forall k\in[1\dots L-1], \forall x \in X_{k} 
		\\
		P^{q} = P,
	\end{cases}
	\]
	where $P$ is the transition function of the CMDP and $P^q$ is the one induced by $q$ (see Equation~\eqref{eq:induced_trans}).
\end{lemma}


Notice that any valid occupancy measure $q$ induces a transition function $P^{q}$ and a policy $\pi^{q}$ as:
\begin{equation}P^{q}(x^{\prime}|x,a)= \frac{q(x,a,x^{\prime})}{q(x,a)}   \quad \text{and} \quad \pi^{q}(a|x)=\frac{q(x,a)}{q(x)}.\label{eq:induced_trans}
\end{equation}

\subsection{Performance metrics to evaluate learning algorithms}

In order to define the performance metrics used to evaluate our \emph{online} learning algorithms, we need to introduce an \emph{offline} optimization problem.
%
Given a CMDP with transition function $P$, we define the following parametric \emph{linear program} (Program~\eqref{lp:offline_opt}), which is parametrized by a reward vector $r \in [0,1]^{|X \times A|}$, a constraint cost matrix $G \in [0,1]^{|X \times A| \times m}$ and a threshold vector ${\alpha} \in [0,L]^m$.
\begin{equation}\label{lp:offline_opt}
		\text{OPT}_{r, G, {\alpha}} \coloneqq \begin{cases}
		\max_{q \in \Delta(P)} & r^{\top}  q \quad \text{s.t.}\\
		 & G^{\top}  q \leq  {\alpha} ,
	\end{cases}
\end{equation}
where $ q\in[0,1]^{|X\times A|}$ is a vector encoding an occupancy measure, whose values are defined for state-action pairs according to Equation~\eqref{def:q vector}, and $\Delta(P)$ is the set of all valid occupancy measures given the transition function $P$ (this set can be encoded by linear constraints thanks to Lemma~\ref{lem:occupancy_rosenberg}).

We say that an instance of Program~\eqref{lp:offline_opt} satisfies \emph{Slater's condition} if the following holds.
%
\begin{condition}[Slater]\label{cond:slater}
	There exists an occupancy measure $q^\circ\in\Delta(P)$ such that $G^\top q^\circ < \alpha$.
\end{condition}
%
Moreover, we also introduce a problem-specific \emph{feasibility parameter} related to Program~\eqref{lp:offline_opt}. This is denoted by $\rho\in[0,L]$ and formally defined as
$
	\rho \coloneqq \sup_{q \in \Delta(P)} \min_{i \in [m]} \left[  \alpha-G^\top q \right]_i
$.\footnote{In this paper, given a vector $y$, we denote by $[y]_i$ its $i$-th component.}
%
Intuitively, $\rho$ represents by how much feasible solutions to Program~\eqref{lp:offline_opt} strictly satisfy the constraints.
%
% represents the minimum satisfaction of the constraints attained by a strictly feasible solution $q^\circ$.
%
Notice that Condition~\ref{cond:slater} is equivalent to say that $\rho > 0$, while, whenever $\rho = 0$, there is no occupancy measure that allows to strictly satisfy the constraints $G^{\top}  q \leq  \alpha$ in Program~\eqref{lp:offline_opt}.
%
%In the second part of the paper, namely, when the corruption is unknown (see Section~\ref{sec: unknown_C}), we will make use of the following assumption.
%\begin{assumption}
%	Condition~\ref{cond:slater} holds, namely, it holds that $\rho>0$.
%\end{assumption}
%\stradi{forse dovremmo dire che useremo la $\rho$ di $\text{OPT}_{\overline{r}, \overline{G}, \underline{\alpha}}$, ma non so dove}


We are now ready to introduce the notion of \emph{(cumulative) regret} and \emph{positive (cumulative) constraint violation}, which are the performance metrics that we use to evaluate our learning algorithm.
%
In particular, we define the cumulative regret over $T$ episodes as follows:
\begin{equation*}
	R_{T} \coloneqq  T \cdot\text{OPT}_{\overline{r}, \overline{G}, \alpha}-  \sum_{t\in[T]}  \mathbb{E}[r_{t}]^{\top}   q^{P, \pi_{t}}  ,
\end{equation*}
where  $\overline{r} \coloneqq 
\frac{1}{T}\sum_{t=1}^{T}  \mathbb{E}[r_{t}]  $ and $\overline{G} \coloneqq 
\frac{1}{T}\sum_{t=1}^{T}  \mathbb{E}[G_t]$.
%
%$\overline{G}$ is such that
%$\left[\overline{G}\right]_i:= 
%\frac{1}{T}\sum_{t=1}^{T}  \mathbb{E}[g_{t,i}],$ for all $i \in [m]  $.
%
% Notice that the regret is computed with respect to an \emph{optimal safe occupancy in hindsight}.
%
In the following, we denote by $q^*$ an occupancy measure solving Program~\eqref{lp:offline_opt} instantiated with $\overline{r}$, $\overline{G}$, and $\alpha$, while its corresponding policy (computed by Equation~\eqref{eq:induced_trans}) is $\pi^*$.
%
Thus, $\text{OPT}_{\overline{r}, \overline{G}, \alpha}=\overline{r}^{\top} q^*$ and the regret is $R_T \coloneqq \sum_{t=1}^T \mathbb{E}[r_t]^\top (q^*-q^{P,\pi_t})$.
%
Furthermore, we define the positive cumulative constraint violation over $T$ episodes as:
\begin{equation*}
	V_{T}:= \max_{i\in[m]}\sum_{t\in[T]}\left[ \mathbb{E}[G_t]^{\top} q^{P,\pi_{t}}-{\alpha}\right]^+_i,
\end{equation*}
where we let $[\cdot]^+:=\max\{0, \cdot\}$.
%
% Notice that, in our definition of $V_T$, constraint violations are \emph{not} allowed to cancel out across episodes. This is a much more demanding performance metric than those employed in~\citep{ding_non_stationary,wei2023provably}, which instead allow for cancellations.
%
In the following, for ease of notation, we compactly refer to $q^{P,\pi_{t}}$ as $q_t$, thus omitting the dependency on $P$ and $\pi$. 


\begin{remark}[Relation with adversarial/stochastic CMDPs]
%
Our setting is more akin to CMDPs with adversarial rewards and constraints, rather than stochastic ones.
%
This is because our notion of regret is computed with respect to an optimal constraint-satisfying policy in hindsight that takes into account the average over episodes of the mean values $\mathbb{E}[r_{t}]$ and $\mathbb{E}[G_t]$ of the adversarially-selected probability distributions $\mathcal{R}_t$ and $\mathcal{G}_t$.
%
This makes our setting much harder than one with stochastic rewards and constraints.
%
Indeed, in the special case in which the supports of $\mathcal{R}_t$ and $\mathcal{G}_t$ are singletons (and, thus, mean values are fully revealed after each episode), our setting reduces to a CMDP with adversarial rewards and constraints, given that such supports are selected adversarially.
%
%The careful reader will notice that our setting employs adversarial baselines (e.g. the optimal occupancy in hindsight), while taking the expectation of the rewards/cost for each episode. This is done since, our setting is much harder than the standard stochastic one: indeed, even ignoring the stochasticity of the samples at each episode -- that is, even if the mean values of reards/costs were revealed at each episode --, our setting would be harder that online stochastic MDPs given the adversarial nature of the mean values.
%
\end{remark}

\begin{remark}[Impossibility results carrying over from adversarial CMDPs]
	\citet{Mannor} show that, in online learning problems with constraints selected adversarially, it is impossible to achieve both regret and constraint violation growing sublinearly in $T$.
	%
	This result holds for a regret definition that corresponds to ours. Thus, it carries over to our setting.
	%
	This is why we look for algorithms whose regret and positive constraint violation scale as $\tilde{\mathcal{O}}(\sqrt{T}+C)$, with a linear dependency on the adversarial corruption $C$.
	%
	Notice that the impossibility result by~\citet{Mannor} does not rule out the possibility of achieving such a guarantee, since regret and positive constraint violation are not sublinear when $C$ grows linearly in $T$, as it could be the case in a classical adversarial setting. 
\end{remark}
%
%Given the impossibility result shown by~\citet{Mannor}, that is, the impossibility to achieve both sublinear\footnote{We say that a performance metric is sublinear in $T$, if it is equal to $o(T)$.} regret and violations when the constraints are chosen adversarially and \emph{employing our baseline}, our goal is to achieve sublinear regret and violations bounds which scale linearly with respect to the adversariality (corruption) of the environment. Precisely, in Section~\ref{sec: known_c}, we propose an algorithm which achieves $\BigOL{\sqrt{T}+C}$ regret and violations when the true corruption value is known.
%Finally, in Section~\ref{sec: unknown_C} we propose an algorithm which builds on top the aforementioned one and attains $\BigOL{\sqrt{T}+C}$ regret and violations when the corruption value is \emph{not} known. Please notice that ou bounds are not sublinear only for $C=\Theta(T)$, thus being coherent with the lower bound of~\citep{Mannor}.
